ELIGN: Expectation Alignment as a Multi-Agent Intrinsic Reward

Modern multi-agent reinforcement learning frameworks rely on centralized training and reward shaping to perform well. However, centralized training and dense rewards are not readily available in the real world. Current multi-agent algorithms struggle to learn in the alternative setup of decentralized training or sparse rewards. To address these issues, we propose a self-supervised intrinsic reward ELIGN - expectation alignment - inspired by the self-organization principle in Zoology. Similar to how animals collaborate in a decentralized manner with those in their vicinity, agents trained with expectation alignment learn behaviors that match their neighbors' expectations. This allows the agents to learn collaborative behaviors without any external reward or centralized training. We demonstrate the efficacy of our approach across 6 tasks in the multi-agent particle and the complex Google Research football environments, comparing ELIGN to sparse and curiosity-based intrinsic rewards. When the number of agents increases, ELIGN scales well in all multi-agent tasks except for one where agents have different capabilities. We show that agent coordination improves through expectation alignment because agents learn to divide tasks amongst themselves, break coordination symmetries, and confuse adversaries. These results identify tasks where expectation alignment is a more useful strategy than curiosity-driven exploration for multi-agent coordination, enabling agents to do zero-shot coordination.

==> figures/centralized_fo.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/centralized_fo_rew.png}
    \caption{We plot the test episode rewards of centralized algorithms under full observability}
    \label{fig:centralized_fo}
\end{figure*}


==> figures/centralized_po.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/centralized_po_occupancy.png}
    \caption{We plot the test episode occupancy/collision count of \textit{centralized} algorithms under partial observability. Both centralized $\textrm{\textsc{elign}}_\textrm{self}$ and $\textrm{\textsc{elign}}_\textrm{team}$ outperform \textsc{sparse} in cooperative tasks \textit{Coop nav (5v0)} and \textit{Hetero nav (6v0)}. Either $\textrm{\textsc{elign}}_\textrm{team}$ or $\textrm{\textsc{elign}}_\textrm{adv}$ beats \textsc{sparse} in competitive tasks.}
    \label{fig:centralized_po_occ}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/centralized_po_rew.png}
%     \caption{We plot the test episode rewards of centralized algorithms under partial observability}
%     \label{fig:centralized_po}
% \end{figure*}



==> figures/dec_occ_large.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/dec_occ_large.pdf}
    \vspace{-1em}
    \caption{We plot the average test occupancy/collision count per step of decentralized algorithms in all tasks when the number of agents is doubled. }
    \label{fig:dec_occ_large}
\end{figure*}

==> figures/gfootball_env.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/gfootball_3v1_keeper.png}
%     \caption{An illustration of the Academy 3 vs 1 with Keeper scenario from the Google research football environment.}
%     \label{fig:gfootball_env}
% \end{figure}
% for neurips

% \begin{wrapfigure}[15]{R}{0.5\linewidth}
%     \centering
%     \vspace{-1\intextsep}
%     \hspace*{-.75\columnsep}\includegraphics[width=\linewidth]{figures/gfootball_3v1_keeper.png}
%     \caption{An illustration of the Academy 3 vs 1 with Keeper scenario from the Google research football environment.}
%     \label{fig:gfootball_env}
% \end{wrapfigure}

==> figures/symmetry_fo.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/symmetry_breaking_bar_plots_fo.png}
    \caption{We plot the test episode rewards of in symmetry-breaking settings under full observability}
    \label{fig:symmetry_fo}
\end{figure*}


==> tables/1_dec_reward_icml.tex <==
\begin{table*}[t]
\centering 
\caption{\label{tab:1_dec_reward}We report the mean test episode extrinsic rewards and standard errors of $\textit{decentralized}$ methods with different intrinsic rewards under partial and full observability. Under partial observability, $\textrm{\textsc{align}}_\textrm{self/team/adv}$ outperforms \textsc{sparse} and both curiosity-based intrinsic rewards $\textrm{\textsc{curio}}_\textrm{self,team}$ on all tasks. Under full observability, $\textrm{\textsc{align}}_\textrm{team}$ mostly surpasses $\textsc{sparse}$ and $\textrm{\textsc{curio}}_\textrm{self}$ except for $\textit{Keep-away (2v2)}$ and $\textit{Physical deception (2v1)}$ respectively. These results demonstrate the benefit of using alignment as intrinsic reward to train better decentralized policies, especially under partial observability.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{llrp{0.001pt}rp{0.001pt} rp{0.001pt}rp{0.001pt}r}
\multicolumn{2}{l}{}                & \multicolumn{3}{c}{\textbf{Cooperative}}                              & & \multicolumn{5}{c}{\textbf{Competitive}}                                                                            \\
\cmidrule{3-5}\cmidrule{7-11}
\multicolumn{2}{l}{Task (Agt \# vs. Adv \#) }                & \multicolumn{1}{c}{\textbf{Coop nav. (3v0)}} && \multicolumn{1}{c}{\textbf{Hetero nav. (4v0)}} && \multicolumn{1}{c}{\textbf{Phy decep. (2v1)}}  && \multicolumn{1}{c}{\textbf{Pred-prey (2v2)}} && \multicolumn{1}{c}{\textbf{Keep-away (2v2)}} \\
\cmidrule{1-2}\cmidrule{3-3}\cmidrule{5-5}\cmidrule{7-7}\cmidrule{9-9}\cmidrule{11-11}
\multirow{6}{*}{\textbf{Partial observability}} & $\textsc{sparse}^1$                & $139.07\pm 13.63$           && $284.42\pm 12.83$ && $93.60\pm 8.61$ && $-4.72\pm 2.4$ && $4.58\pm 3.27$ \\
                         &  $\textrm{\textsc{curio}}_\textrm{self}^2$        & $133.93\pm 7.66$            && $286.22\pm  9.97$             && $68.80\pm  7.93$                 && $-6.50\pm  2.18$             && $11.88\pm2.88$            \\
                         & $\textrm{\textsc{curio}}_\textrm{team}^3$           & $125.42\pm11.95$           && $262.28\pm22.59$            && $85.31\pm 11.93$                && $-3.57\pm 1.75$              && $9.54\pm 5.04$\\
                         & $\textrm{\textsc{align}}_\textrm{self}$        & $\mathbf{155.88}\pm \mathbf{5.11} $          && $292.34\pm 9.24$             && $69.91\pm 4.51$                 && $-7.58\pm2.55$              && $12.84\pm 4.29$            \\
                         & $\textrm{\textsc{align}}_\textrm{team}$   & $141.04\pm            8.04$            && $\mathbf{311.67}\pm            \mathbf{10.88}$           && $\mathbf{101.72}\pm \mathbf{6.31}$                 && $-7.69\pm 2.69$              && $2.96\pm 4.03$                       \\
                         & $\textrm{\textsc{align}}_\textrm{adv}$      & ---         && ---               && $92.20\pm 4.23$                 && $\mathbf{-2.51}\pm \mathbf{1.70}$              && $\mathbf{19.46}\pm \mathbf{5.05}$ \\
                        %  & \textrm{\textsc{align}}_\textrm{both}   & ---            && ---            && 92.13\pm 11.81                && \mathbf{-1.89}\pm \mathbf{1.50}              && 3.50\pm1.84                     \\
                         \hline
\multirow{3}{*}{\textbf{Full observability}}    & $\textsc{sparse}^1$      & $154.00\pm10.51$           && $274.75\pm19.74$            && $82.97\pm 12.23$                && $-10.48\pm 4.20$              && $\mathbf{4.95}\pm \mathbf{2.96}$            
                         \\
                         & $\textrm{\textsc{curio}}_\textrm{self}$   & $154.71\pm 8.00$            && $268.85\pm 15.61$            && $\mathbf{100.66}\pm \mathbf{15.14}$                && $-8.74\pm4.62$              && $-2.00\pm 1.24$            \\
                         & $\textrm{\textsc{align}}_\textrm{self}$ &  $\mathbf{161.70}\pm \mathbf{4.52}$            && $\mathbf{280.16}\pm\mathbf{17.12}$           && $87.50 \pm 15.40$                && $\mathbf{-5.60}\pm \mathbf{2.60}$              && $0.40\pm 1.92$ \\
                        \multicolumn{11}{l}{$^1$~\cite{lowe2017multi},$^2$~\cite{stadie2015incentivizing},$^3$~\cite{iqbal2020coordinated}}  
\end{tabular}
}
\end{table*}


==> tables/2_dec_reward_gfootball.tex <==
\begin{table*}[t]
\centering 
{\renewcommand{\arraystretch}{0.5}
\caption{\label{tab:2_dec_reward_gfootball} We report the mean average episode rewards and standard errors of the algorithms in the \textit{Academy 3vs1 with keeper} task of the Google Research football environment. $\textrm{\textsc{elign}}_\textrm{adv}$ achieves the best performance among all reward types.}
\begin{small}
\begin{tabular}{ll} 
\toprule
Method & Mean avg. episode reward   \\ \midrule
 $\textsc{sparse}^1$ & $0.020\pm0.001$ \\
 $\textrm{\textsc{curio}}_\textrm{self}$  & $0.024\pm0.004$ \\
  $\textrm{\textsc{curio}}_\textrm{team}$  & $0.021\pm0.002$ \\
  $\textrm{\textsc{elign}}_\textrm{self}$  & $0.003\pm0.018$ \\
 $\textrm{\textsc{elign}}_\textrm{team}$  & $0.022\pm 0.001$ \\
  $\textrm{\textsc{elign}}_\textrm{adv}$  & $\mathbf{0.025}\pm\mathbf{0.001}$ \\ 
\bottomrule
 {$^1$~\cite{kurach2019gfootball}} 
\end{tabular}
 \end{small}
}
\end{table*}

==> tables/2_scaled_dec_reward_icml.tex <==
\begin{table*}[t]
\centering 
\caption{\label{tab:2_scaled_dec_reward}We report the mean test episode extrinsic rewards and standard errors of $\textit{decentralized}$ methods with different intrinsic rewards in $\textit{scaled}$ environments. Under partial observability, both $\textrm{\textsc{align}}_\textrm{self,team}$ outperform $\textsc{sparse}$ in cooperative tasks. One of $\textrm{\textsc{align}}_\textrm{self,team,adv}$ always achieves the best performance in competitive tasks. With full observability, $\textrm{\textsc{align}}_\textrm{self}$ beats \textsc{sparse} across all tasks.
}
\resizebox{\textwidth}{!}{
\begin{tabular}[width=\linewidth]{llrp{0.001pt}rp{0.001pt} rp{0.001pt}rp{0.001pt}r}
\multicolumn{2}{l}{}                & \multicolumn{3}{c}{\textbf{Cooperative}}                              & & \multicolumn{5}{c}{\textbf{Competitive}}                                                                            \\
\cmidrule{3-5}\cmidrule{7-11}
\multicolumn{2}{l}{Task (Agt \# vs. Adv \#) }                & \multicolumn{1}{c}{\textbf{Coop nav. (5v0)}} && \multicolumn{1}{c}{\textbf{Hetero nav. (6v0)}} && \multicolumn{1}{c}{\textbf{Phy decep. (4v2)}}  && \multicolumn{1}{c}{\textbf{Pred-prey (4v4)}} && \multicolumn{1}{c}{\textbf{Keep-away (4v4)}} \\
\cmidrule{1-2}\cmidrule{3-3}\cmidrule{5-5}\cmidrule{7-7}\cmidrule{9-9}\cmidrule{11-11}
\multirow{4}{*}{\textbf{Partial observability}} & $\textsc{sparse}^1$             & $459.92\pm22.44$ && $616.62\pm25.30$ && $166.89\pm27.72$ && $-28.75\pm7.3$ && $0.75\pm1.82$        \\
                        &  $\textrm{\textsc{curio}}_\textrm{self}^2$        & $458.45\pm19.79$ && $\mathbf{702.73}\pm\mathbf{18.57}$ && $146.55\pm29.05$ && $-25.35\pm6.16$ && $10.52\pm5.48$            \\
                         & $\textrm{\textsc{curio}}_\textrm{team}^3$           &$497.15\pm11.47$ && $695.38\pm12.22$ && $84.66\pm16.94$ && $-17.21\pm8.23$ && $1.40\pm2.06$\\
                               & $\textrm{\textsc{align}}_\textrm{self}$             & $\mathbf{498.24}\pm\mathbf{9.77}$ && $646.70\pm23.25$ && $137.38\pm30.00$ && $\mathbf{-9.14}\pm\mathbf{5.57}$ && $9.83\pm11.22$       \\
                               & $\textrm{\textsc{align}}_\textrm{team}$       & $488.83\pm20.82$ && $638.74\pm28.93$ && $\mathbf{186.83}\pm\mathbf{21.92}$ && $-20.4\pm5.93$ && $2.07\pm4.55$          \\
                               & $\textrm{\textsc{align}}_\textrm{adv}$          & --- && --- && $182.61\pm17.63$ && $-21.37\pm7.02$ && $\mathbf{11.29}\pm\mathbf{9.02}$       \\
                            %   & $\textrm{\textsc{align}}_\textrm{both}$       & --- && --- && 153.49\pm19.34 && -22.95\pm7.4 && -2.02\pm4.25          \\
                               \hline
\multirow{2}{*}{\textbf{Full observability}} & $\textsc{sparse}^1$    & $523.71\pm34.56$ && $533.67\pm23.28$ && $262.93\pm31.88$ && $-64.35\pm8.71$ && $-2.31\pm2.45$          \\
                               & $\textrm{\textsc{align}}_\textrm{self}$ & $\mathbf{545.35}\pm\mathbf{19.28}$ && $\mathbf{547.27}\pm\mathbf{18.73}$ && $\mathbf{285.64}\pm\mathbf{16.08}$ && $\mathbf{-45.02}\pm\mathbf{7.46}$ && $\mathbf{-2.01}\pm\mathbf{3.53}$    \\
                               \multicolumn{11}{l}{$^1$~\cite{lowe2017multi}} 
\end{tabular}
}
\end{table*}


==> tables/3_central_reward_po.tex <==
\begin{table*}[t]
\centering 
\caption{\label{tab:2_central_rew_po}We report the mean test episode extrinsic rewards and standard errors of $\textit{centralized}$ algorithms trained with different intrinsic rewards under partial observability. In cooperative tasks, either $\textrm{\textsc{elign}}_\textrm{self}$ or $\textrm{\textsc{elign}}_\textrm{team}$ outperforms all other intrinsic reward baselines. Among competitive tasks, $\textrm{\textsc{elign}}_\textrm{self,team,adv}$ all beat the other baselines in \textit{Predator-prey (2v2)} but not \textit{Physical deception (2v2)} or \textit{Keep-away (2v2)}, suggesting that alignment might not provide additional useful signals to centralized algorithms in competitive settings.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{llrp{0.001pt}rp{0.001pt} rp{0.001pt}rp{0.001pt}r}
\multicolumn{2}{l}{}                & \multicolumn{3}{c}{\textbf{Cooperative}}                              & & \multicolumn{5}{c}{\textbf{Competitive}}                                                                            \\
\cmidrule{3-5}\cmidrule{7-11}
\multicolumn{2}{l}{Task (Agt \# vs. Adv \#) }                & \multicolumn{1}{c}{\textbf{Coop nav. (3v0)}} && \multicolumn{1}{c}{\textbf{Hetero nav. (4v0)}} && \multicolumn{1}{c}{\textbf{Phy decep. (2v1)}}  && \multicolumn{1}{c}{\textbf{Pred-prey (2v2)}} && \multicolumn{1}{c}{\textbf{Keep-away (2v2)}} \\
\cmidrule{1-2}\cmidrule{3-3}\cmidrule{5-5}\cmidrule{7-7}\cmidrule{9-9}\cmidrule{11-11}
\multirow{6}{*}{\textbf{Partial observability}} & \textsc{sparse}$^1$                & $113.25\pm8.10 $ && $ 178.62\pm9.62 $ && $ \mathbf{117.45}\pm\mathbf{10.63} $ && $ -1.96\pm1.45 $ && $ \mathbf{35.79}\pm\mathbf{14.93} $\\
                         &  $\textrm{\textsc{curio}}_\textrm{self}^2$        & $128.77\pm7.70 $ && $ 190.30\pm7.73 $ && $ 111.08\pm10.09 $ && $ -1.63\pm1.27 $ && $ 13.94\pm12.56 $           \\
                         & $\textrm{\textsc{curio}}_\textrm{team}^3$           & $114.13\pm11.84 $ && $ 189.80\pm11.81 $ && $ 114.32\pm5.46 $ && $ -3.04\pm1.09 $ && $ 6.01\pm3.36$\\
                         & $\textrm{\textsc{elign}}_\textrm{self}$        & $\mathbf{137.14}\pm\mathbf{3.63} $ && $ 169.58\pm14.99 $ && $ 93.27\pm3.70 $ && $ -0.41\pm0.28 $ && $ 22.77\pm9.91$            \\
                         & $\textrm{\textsc{elign}}_\textrm{team}$  & $119.10\pm10.89 $ && $ \mathbf{210.81}\pm\mathbf{9.70} $ && $ 96.49\pm6.46 $ && $ -0.92\pm0.72 $ && $ 24.94\pm12.58 $                     \\
                         & $\textrm{\textsc{elign}}_\textrm{adv}$      & ---          &&  ---                && $ 102.37\pm6.98 $ && $ \mathbf{-0.13}\pm\mathbf{0.03} $ && $ 8.70\pm4.44 $\\
                         \multicolumn{11}{l}{$^1$~\cite{lowe2017multi},$^2$~\cite{stadie2015incentivizing},$^3$~\cite{iqbal2020coordinated}} 
                        %  & \textrm{\textsc{elign}}_\textrm{both}   & ---            && ---            && 92.13\pm 11.81                && \mathbf{-1.89}\pm \mathbf{1.50}              && 3.50\pm1.84                     \\
\end{tabular}
}
\end{table*}


==> tables/amb_fo_other_metrics.tex <==
\begin{table*}[t]
\centering

\caption{\label{tab:amb_fo_metric_1}  
% Test number of occupancies/collisions per episode for 5 tasks in a \textbf{fully} observable environment with \textbf{ambiguous initialization} . 
    Occupancy and collision metrics averaged across test episodes under the \textit{fully} observable symmetry-breaking setting. Higher scores are better for the occupancy metric ($\uparrow$), and lower scores are better for the collision metric ($\downarrow$). 
}
 \scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$}  && \multicolumn{2}{c}{collision $\downarrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     & 0.449          & 0.648        && \textbf{0.543}         & 0.350         && 0.719              & 0.893             && 0.030           & 0.126           && 0.032         & 0.000         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{0.548}          & \textbf{0.676}        && 0.542         & \textbf{0.548}         && 0.722              & \textbf{0.997}             && 0.009           & \textbf{0.068}           && 0.004         & 0.012         \\
                               & \textsc{shaped}      & 0.222          & 0.112        && 0.330         & 0.128         && \textbf{0.761}              & 0.222             && \textbf{0.004}           & 0.088           && \textbf{1.010}         & \textbf{1.389}         \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     & 0.455          & \textbf{0.270}        && 0.231         & \textbf{0.249}         && 0.747              & \textbf{0.494}             && 0.005           &    0.044             && 0.000         & 0.014         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{0.527}          & 0.108        && \textbf{0.537}         &   0.008            && \textbf{0.975}              & 0.175             && \textbf{0.000}           & \textbf{0.002}           && 0.005         & 0.028         \\
                               & \textsc{shaped}      & 0.430          & 0.083        && 0.055         &    0.154           && 0.713              & 0.251             && 0.006           & 0.029           && \textbf{0.764}         & \textbf{0.656}        
\end{tabular}
}

\end{table*}

\begin{table*}[t]
\centering
\caption{\label{tab:amb_fo_metric_2}  
    % Test mean distance between agents and targets/adversaries per episode for 5 tasks in a \textbf{fully} observable environment with \textbf{ambiguous initialization.}
     Agent-to-target (agt-target) and agent-to-adversary (agt-adv) distances averages across test episodes under the \textit{fully} observable, symmetry-breaking setting. Lower scores are better for agt-target ($\downarrow$), and higher scores are better for agt-adv ($\uparrow$).
 }
 \scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$}  && \multicolumn{2}{c}{agt-adv dist $\uparrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     & 0.407             & 0.211           && 0.296            & 0.427            && 0.260              & \textbf{0.260}             && 1.125           & 1.922           && 1.458            & 3.699            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{0.241}             & \textbf{0.205}           && \textbf{0.293}            & \textbf{0.291}            && 0.272              & \textbf{0.260}             && 1.463           & \textbf{2.318}           && 1.658            & 3.388            \\
                               & \textsc{shaped}      & 0.426             & 0.372           && 0.378            & 0.443            && \textbf{0.213}              & 0.435             && \textbf{1.719}           & 2.161           && \textbf{0.457}            & \textbf{1.011}            \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     & \textbf{0.262}             & \textbf{0.324}           && 0.467            & \textbf{0.548}            && 0.254              & \textbf{0.448}             && 1.563           &             2.524    && 1.911            & 3.200            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & 0.278             & 0.402           && \textbf{0.311}            &        0.714          && \textbf{0.238}              & 0.483             && \textbf{1.810}           & 2.397           && 1.621            & 3.404            \\
                               & \textsc{shaped}      & 0.275             & 0.420           && 0.562            &   0.562               && 0.264              & 0.531             && 1.777           & \textbf{2.694}           && \textbf{0.500}            & \textbf{1.370}      
\end{tabular}
}

\end{table*}


==> tables/amb_fo_test_reward.tex <==
\begin{table*}[t]
\centering
\caption{% 
\label{tab:amb_fo_test_reward} Test episode rewards on decentralized and centralized training under the \textit{fully} observable symmetry-breaking setting. Higher rewards are better. }
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn\textsc{elign}{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical Deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     & 148.400       & 433.739      && 232.395       & \textbf{483.673}       && 80.909             & 188.895           && -8.353          & -27.000         && -0.928       & -6.167         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$ & \textbf{151.167}       & \textbf{511.503}      && \textbf{280.536}       & 482.675      & & 71.627             & \textbf{210.280}           && -3.406        & -16.389         && -1.833       & \textbf{-5.534}         \\
                               & \textsc{shaped}     & 55.977        & 57.472       && 205.071       & 240.288      && \textbf{117.000}            & 24.016            && \textbf{-2.341}          & \textbf{-14.239}         && \textbf{40.091}       & -46.929        \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     & 114.000       & 118.949      && 64.800        & \textbf{98.085}        && 69.000             & -64.969           && -6.000          &    -8.09            && 0.000        & -5.500         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$ & \textbf{169.920}       & \textbf{126.503}      && \textbf{105.600}       &  85.45             && 104.000            & -98.415           && \textbf{0.00}           & \textbf{-0.017}          && -2.500       & \textbf{-5.000}         \\
                               & \textsc{shaped}     & 92.357        & 107.597      && 24.666        &         84.831      && \textbf{162.333}            & \textbf{48.841}            && -1.100          & -7.105          && \textbf{26.691}       & -134.774      
\end{tabular}
}
\end{table*}

==> tables/amb_po_other_metrics.tex <==
\begin{table*}[t]
    \centering
    \caption{\label{tab:amb_po_metric_1}
    % Test number of occupancies/collisions per episode for 5 tasks in a \textbf{partially} observable environment with \textbf{ambiguous initialization}.
    Occupancy and collision metrics averaged across test episodes under the \textit{partially} observable symmetry-breaking setting. Higher scores are better for the occupancy metric ($\uparrow$), and lower scores are better for the collision metric ($\downarrow$). 
    }
    \scalebox{0.85}{
 \begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$}  && \multicolumn{2}{c}{collision $\downarrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline

\multirow{5}{*}{Decentralized} & \textsc{sparse}      & 0.235          & 0.309        && 0.248         & 0.422         && \textbf{0.597}              & 0.748            & & 0.009           & 0.128           && 0.002         & 0.053         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & \textbf{0.322}          & \textbf{0.379}        && \textbf{0.305}         & \textbf{0.459}         && \textbf{0.565}              & 0.709             && 0.019           & 0.095           && 0.076         & 0.083         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---           & ---         && ---          & ---          && 0.589              & 0.742             && 0.008           & 0.063           && 0.184         & 0.038         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$  & ---           & ---         && ---          & ---          && 0.563              & 0.644             && 0.032           & 0.080           && 0.000         & 0.011         \\
                               & \textsc{shaped}       & 0.304          & 0.211        && 0.243         & 0.025         && 0.305              & \textbf{0.984}             && \textbf{0.001}           & \textbf{0.009}           && \textbf{1.062}         & \textbf{1.438}         \\\hline
\multirow{4}{*}{Centralized}   & \textsc{sparse}      & 0.129          &              && 0.169         & 0.001         && 0.521              & \textbf{0.335}            & & 0.001           & \textbf{0.006}           && 0.000         & 0.003         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & \textbf{0.194}          & \textbf{0.219}        && \textbf{0.230}         & \textbf{0.060}         && 0.567              & 0.291             && \textbf{0.000}           & 0.073           && 0.047         & 0.001         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---           & ---         && ---          & ---          && \textbf{1.042}              & 0.315             && \textbf{0.000}           & 0.078           && \textbf{0.333}         & 0.001         \\
                               & \textsc{shaped}       & 0.182          & 0.087        && 0.069         & 0.046        && 0.506              & 0.219             && 0.001           & 0.036           && 0.039         & \textbf{0.466}               
\end{tabular}
}
\end{table*}


\begin{table*}[t]
    \centering
     \caption{\label{tab:amb_po_metric_2} 
     Agent-to-target (agt-target) and agent-to-adversary (agt-adv) distances averages across test episodes under the \textit{partially} observable, symmetry-breaking setting. Lower scores are better for agt-target ($\downarrow$), and higher scores are better for agt-adv ($\uparrow$).
    %  Test mean distance between agents and targets/adversaries per episode for 5 tasks in a \textbf{partially} observable environment with \textbf{ambiguous initialization}.
     }
    \scalebox{0.85}{
    \begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$}  && \multicolumn{2}{c}{agt-adv dist $\uparrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{5}{*}{Decentralized} & \textsc{sparse}      & 0.521             & \textbf{0.378}           && 0.598            & 0.381            && 0.365              & 0.355             && 1.550           & 2.112           && 1.730            & 2.960            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & 0.587             & 0.439           && \textbf{0.521}            & \textbf{0.368}            && \textbf{0.342}              & 0.377             && 1.384           & 2.158           && 1.426            & 2.780            \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---              & ---            && ---             & ---             && 0.364              & 0.337             && 1.550           & 2.386           && 0.940            & 2.902            \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$  & ---              & ---            && ---             & ---             && 0.358              & 0.410             && 1.352           & 2.233           && 1.750            & 3.444            \\
                               & \textsc{shaped}       & \textbf{0.498}             & 0.492           && 0.581            & 0.557            && 0.423              & \textbf{0.287}             && \textbf{1.828}           & \textbf{2.889}          && \textbf{0.452}            & \textbf{1.004}            \\\hline
\multirow{4}{*}{Centralized}   & \textsc{sparse}      & 0.648             &        0.697         && 0.623            & 0.779            && 0.442              & \textbf{0.390}             && 1.524           & 2.548           && 1.911            & 3.676            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & 0.581             & \textbf{0.421}           && \textbf{0.553}            & 0.672            && 0.346              & 0.530            & & 1.694           & 2.456           && 1.367            & 3.703            \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---              & ---            && ---             & ---             && \textbf{0.257}              & 0.396             && 1.685           & 2.507           && \textbf{1.025}            & 3.653            \\
                               & \textsc{shaped}       & \textbf{0.548}             & 0.502           && 0.664            & 0.565      && 0.383              & 0.782             && \textbf{1.754}           & \textbf{2.675}          & & 1.272            & \textbf{1.853}    
         
\end{tabular}
}
   
\end{table*}


==> tables/amb_po_test_reward.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:amb_po_test_reward} Test episode rewards on decentralized and centralized training under the \textit{partially} observable symmetry-breaking setting. Higher rewards are better.}
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical Deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}   & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline

\multirow{5}{*}{Decentralized} & \textsc{sparse}      & 95.353        & 304.632      && 184.319       & \textbf{420.407}       && 62.655            & 197.243            && \textbf{0.000}           & -30.000         && -1.000        & 3.766         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{111.152}       & \textbf{361.664}      && \textbf{203.356  }     & 386.536       && 78.831            & 207.484           && -3.250          & -23.956         && 5.444         & \textbf{8.578}         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$  & ---          & ---         && ---          & ---          && \textbf{94.318}            & 201.784            && -2.330          & -21.003         && 17.198    & 3.516         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$ & ---          & ---         && ---          & ---          && 67.174            & 198.445            && -5.801          & -13.591         && -0.500        & -1.167        \\
                               & \textsc{shaped}       & 94.258        & 234.369      && 129.888       & 129.933       && 60.472            & \textbf{328.000}            && -0.032          & \textbf{-2.288}          && \textbf{74.149}        & -8.879        \\\hline
\multirow{4}{*}{Centralized}   & \textsc{sparse}      & 31.145        &              && 70.185        & 47.251        && 10.351            & -261.437           && -1.000          & \textbf{-0.360}          && 0.000         & -4.500        \\
                               & $\textrm{\textsc{elign}}_\textrm{agt}$  & \textbf{76.235}        & 51.947       && \textbf{98.894}        &      \textbf{50.494}       && 7.000             & -38.924           && -0.213          & -11.037         && -3.714        & \textbf{-3.500}        \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$  & ---          & ---         && ---          & ---          && 77.149            & -139.981           && \textbf{0.000}           & -13.000         && \textbf{38.500}       & \textbf{-3.500}        \\
                               & \textsc{shaped}       & 62.770        & 57.486       && 17.600        &               && \textbf{118.096}           & \textbf{57.486}             && -0.189          & -9.651          && -13.419       & -19.400      
\end{tabular}
}
\end{table*}

==> tables/amb_po_test_reward_centralized.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:amb_po_test_reward_centralized} Test episode rewards on centralized training under the \textit{partially} observable symmetry-breaking setting. Higher rewards are better. }
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{team \# vs. Adv \#}   & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{4}{*}{Centralized}   & \textsc{sparse}      & 31.145        &      0.000        && 70.185        & 47.251        && 10.351            & -261.437           && -1.000          & \textbf{-0.360}          && 0.000         & -4.500        \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{76.235}        & 51.947       && \textbf{98.894}        &      50.494      && 7.000             & -38.924           && -0.213          & -11.037         && -3.714        & \textbf{-3.500}        \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$  & ---          & ---         && ---          & ---          && 77.149            & -139.981           && \textbf{0.000}           & -13.000         && \textbf{38.500}       & \textbf{-3.500}        \\
                               & \textsc{shaped}       & 62.770        & \textbf{66.733}       && 17.600        &     \textbf{90.190}          && \textbf{118.096}           & \textbf{57.486}             && -0.189          & -9.651          && -13.419       & -19.400      
\end{tabular}
}
\end{table*}

==> tables/amb_po_test_reward_decentralized.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:amb_po_test_reward_decentralized}For symmetry-breaking initializations, we find that $\textrm{\textsc{elign}}_\textrm{team}$ improves cooperative tasks. For competitive tasks, hand-designed \textsc{shaped} still outperform others.
% of decentralized training with sparse, alignment and dense rewards in 5 tasks with partial observability and ambiguous initialization. 
}
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical Deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}   & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline

\multirow{5}{*}{Decentralized} & \textsc{sparse}      & 95.353        & 304.632      && 184.319       & \textbf{420.407}       && 62.655            & 197.243            && \textbf{0.000}           & -30.000         && -1.000        & 3.766         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{111.152}       & \textbf{361.664}      && \textbf{203.356  }     & 386.536       && 78.831            & 207.484           && -3.250          & -23.956         && 5.444         & \textbf{8.578}         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$  & ---          & ---         && ---          & ---          && \textbf{94.318}            & 201.784            && -2.330          & -21.003         && 17.198    & 3.516         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$ & ---          & ---         && ---          & ---          && 67.174            & 198.445            && -5.801          & -13.591         && -0.500        & -1.167        \\
                               & \textsc{shaped}       & 94.258        & 234.369      && 129.888       & 129.933       && 60.472            & \textbf{328.000}            && -0.032          & \textbf{-2.288}          && \textbf{74.149}        & -8.879        \\
\end{tabular}
}
\end{table*}

==> tables/fo_other_metrics.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:fo_metric_1}  Occupancy and collision metrics averaged across test episodes under \textit{full} observability. Higher scores are better for the occupancy metric ($\uparrow$), and lower scores are better for the collision metric ($\downarrow$). }
 \scalebox{0.85}{
\begin{tabular}{llp{0.001pt}rrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{3}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{4-8}\cmidrule{10-17}
\multicolumn{2}{l}{Task}                && \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$}  && \multicolumn{2}{c}{collision $\downarrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} \\
\cmidrule{4-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}\cmidrule{16-17}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       && \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     && 0.447          & 0.647        && 0.558         & 0.389         && 0.737              & 0.987             && 0.029           & 0.196           && 0.052         & 0.033         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  && \textbf{0.580}          & \textbf{0.667}        && \textbf{0.559}         & \textbf{0.565}         && 0.731              & \textbf{1.038}             && \textbf{0.009}           & \textbf{0.102}           && 0.023         & 0.051         \\
                               & \textsc{shaped}      && 0.345          & 0.128        && 0.424         & 0.154         && \textbf{0.738}              & 0.285            && 0.010           & 0.146           && \textbf{1.019}         & \textbf{1.514}         \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     && 0.443          & \textbf{0.289}        && 0.312         & \textbf{0.360}        & & 0.782              & \textbf{0.686}             && 0.027           &       0.063          && 0.016         & 0.051         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  && \textbf{0.524}          & 0.125        && \textbf{0.535}         &      0.117         && \textbf{0.935}              & 0.381             && \textbf{0.001}           & \textbf{0.004}           && 0.023         & 0.028         \\
                               & \textsc{shaped}      && 0.456          & 0.092        && 0.115         &       0.144        && 0.718              & 0.336             && 0.018           & 0.042           && \textbf{0.775}         & \textbf{0.736}        
\end{tabular}
}

\end{table*}

\begin{table*}[t]
\centering
\caption{ \label{tab:fo_metric_2}  
Agent-to-target (agt-target) and agent-to-adversary (agt-adv) distances averages across test episodes under \textit{full} observability. Lower scores are better for agt-target ($\downarrow$), and higher scores are better for agt-adv ($\uparrow$).
}
 \scalebox{0.85}{
\begin{tabular}{llp{0.001pt}rrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{3}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{4-8}\cmidrule{10-17}
\multicolumn{2}{l}{Task}                && \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$}  && \multicolumn{2}{c}{agt-adv dist $\uparrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} \\
\cmidrule{4-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}\cmidrule{16-17}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       && \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     && 0.362             & 0.166           && \textbf{0.230}            & 0.309            && 0.271              & 0.209             && 1.114           & 1.600           && 1.367            & 3.288            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  && \textbf{0.224}             & \textbf{0.162}           && \textbf{0.230}            & \textbf{0.206}            && 0.276              & \textbf{0.208}             && 1.392           & \textbf{2.042}           && 1.500            & 3.063            \\
                               & \textsc{shaped}      && 0.322             & 0.294          & & 0.274            & 0.334            && \textbf{0.240}              & 0.416             && \textbf{1.612}           & 1.875           && \textbf{0.572}            & \textbf{1.224}            \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     && 0.242             & \textbf{0.264}           && 0.340            & \textbf{0.298}            && 0.256              & 0.402             && 1.314           &       2.270          && 1.690            & 3.043            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  && 0.256             & 0.318           && \textbf{0.255}            &          0.392        && \textbf{0.245}              & \textbf{0.395}             && \textbf{1.641}           & 2.193           && 1.544            & 3.404            \\
                               & \textsc{shaped}      && \textbf{0.227}             & 0.326           && 0.398            &    0.352              && 0.265              & 0.419             && 1.462           & \textbf{2.514}          && \textbf{0.633}            & \textbf{1.501}           
\end{tabular}
}

\end{table*}

==> tables/fo_test_reward.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:fo_test_reward}We show test episode extrinsic rewards under perfect observability. With decentralized algorithms, $\textrm{\textsc{elign}}_\textrm{team}$ performs the best on most tasks. Similar to the previous table, we find that the decentralized algorithm with $\textrm{\textsc{elign}}_\textrm{team}$ outperforms the centralized algorithm with $\textrm{\textsc{shaped}}$ on all but one task (\textit{predator-prey}).
}
\scalebox{0.83}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{8-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{3}{*}{Decentralized} & \textsc{sparse}     & 154.342       & 493.417      && 243.979       & \textbf{545.153}   &    & 116.430            & 221.012           && -11.052         & -71.835         && 2.644         & -2.500        \\
                              & $\textrm{\textsc{elign}}_\textrm{team}$ & \textbf{159.219}       & \textbf{525.100}      && \textbf{302.612}       & 524.457 && \textbf{117.857}            & \textbf{274.060}           && -3.941          & \textbf{-30.686}         && -0.167        & \textbf{-2.330}        \\
                               & \textsc{shaped}      & 77.341        & 145.309      && 234.237       & 281.955  &     & 97.898             & -26.000           && \textbf{-1.527}          & -30.731         && \textbf{36.749}        & -15.336       \\\hline
\multirow{3}{*}{Centralized}   & \textsc{sparse}     & 129.988       & 102.469      && \textbf{137.767}       & 214.369    &   & 121.122            & -18.996           && -9.094          & -21.068              && -0.500       & \textbf{5.184}         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$ & \textbf{163.481}       & \textbf{125.780}     && 118.242       & 168.025     &        & 100.559            & -10.310           && \textbf{-0.189}          & \textbf{-1.555}       && -2.000        & -5.000        \\
                               & \textsc{shaped}      & 111.411       & 80.986       && 83.295        &  \textbf{297.623}     &      & \textbf{141.864}            & \textbf{116.336}           && -2.050          & -14.943         && \textbf{44.070}        & -88.338      
\end{tabular}
}
\end{table*}

==> tables/po_mixed_eval.tex <==
\begin{table*}[t]
\centering
\caption{\label{tab:po_mixed_eval}Agents trained with $\textrm{\textsc{elign}}_\textrm{team}$ generalize the best with new agents on all but two task conditions (\textit{heterogeneous navigation} 6v0 and \textit{physical deception}, 2v1)
.}
\scalebox{0.8}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{4}{*}{Decentralized} & \textsc{sparse}      & 141.343       & 431.186      && 267.810       & \textbf{701.198}       && \textbf{119.321}            & 237.274           && -0.088          & -44.018         && 1.000         & -3.500        \\
% & $\textrm{\textsc{elign}}_\textrm{self}$ & 160.69	         &       && 139.17	     &       && 111.20               &           & & 	-8.54	         &         && 16.90          & \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$  & \textbf{146.405}       & \textbf{470.321}      && \textbf{269.500}       & 677.644       && 72.065             & \textbf{271.104}           && -8.099          & -50.096         && 11.000        & 3.500         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$  & ---          & ---         && ---          & ---          && 106.258            & 154.445          && \textbf{-0.085}          & \textbf{-25.557}        && \textbf{16.500}       & \textbf{3.557}         \\
                            %   & $\textrm{\textsc{elign}}_\textrm{both}$ & ---          & ---         && ---          & ---          && 45.691             & 248.024          & & -0.096          & -44.905         && 2.500         & -2.809       
\end{tabular}
}
\end{table*}

==> tables/po_mixed_eval_other_metrics.tex <==
\begin{table*}[t]
\centering
\caption{ \label{tab:po_mixed_eval_metric_1} 
% Test number of occupancies/collisions per episode of decentralized agents trained with sparse and alignment rewards. The agents in each group are trained with different seeds and evaluated together on a new seed.
    Occupancy and collision metrics averaged across test episodes under the \textit{partially} observable zero-shot coordination setting. Higher scores are better for the occupancy metric ($\uparrow$), and lower scores are better for the collision metric ($\downarrow$). 
}
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$}  && \multicolumn{2}{c}{collision $\downarrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{4}{*}{Decentralized} & \textsc{sparse}      & 0.291          & \textbf{0.545}       & & \textbf{0.623}         & 0.678         && 0.908              & 1.271             && \textbf{0.000}           & 0.137           && 0.034         & 0.062         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & \textbf{0.541}          & 0.405        && \textbf{0.623}         & \textbf{0.685}         && 0.773              & 1.195             && 0.022           & 0.131           && 0.113         & \textbf{0.142}         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---           & ---         && ---          & ---          && \textbf{0.918}              & 1.096             && 0.001           & \textbf{0.086}           && \textbf{0.133}         & 0.084         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$  & ---           & ---         && ---          & ---          && 0.883              & \textbf{1.307}             && 0.002           & 0.142           && 0.032         & 0.064      
\end{tabular}
}
\end{table*}

\begin{table*}[t]
\centering
\caption{ \label{tab:po_mixed_eval_metric_2} 
% Test mean distance between agents and targets/adversaries per episode of decentralized agents trained with sparse and alignment rewards in 5 tasks. The agents in each group are trained with different seeds and evaluated together on a new seed.
     Agent-to-target (agt-target) and agent-to-adversary (agt-adv) distances averages across test episodes under the \textit{partially} observable, zero-shot coordination setting. Lower scores are better for agt-target ($\downarrow$), and higher scores are better for agt-adv ($\uparrow$).
}
\scalebox{0.85}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                & \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$}  && \multicolumn{2}{c}{agt-adv dist $\uparrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{4}{*}{Decentralized} & \textsc{sparse}      & \textbf{0.287}             & \textbf{0.281}           && 0.246            & \textbf{0.178}            && 0.288              & 0.217             && 1.392           & 2.091           && 1.589            & 3.189            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$   & \textbf{0.287}             & 0.410           && \textbf{0.234}            & 0.193            && 0.307              & 0.227            & & 1.413           & 2.051           && 1.278            & \textbf{2.671}            \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$    & ---              & ---            && ---             & ---             && \textbf{0.269}              & 0.238             && \textbf{1.435}           & \textbf{2.327}           && \textbf{1.150}            & 2.922            \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$  & ---              & ---            && ---             & ---             && 0.278              & \textbf{0.212}             && 1.370      & 2.019           && 1.566            & 3.092  
\end{tabular}
}
\end{table*}

==> tables/po_other_metrics.tex <==
\begin{table*}[t]
    \centering
    \caption{\label{tab:po_metric_1} Occupancy and collision metrics averaged across test episodes under \textit{partial} observability. Higher scores are better for the occupancy metric ($\uparrow$), and lower scores are better for the collision metric ($\downarrow$). }
    \scalebox{0.85}{
 \begin{tabular}{llp{0.001pt}rrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{3}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{4-8}\cmidrule{10-17}
\multicolumn{2}{l}{Task}                && \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                && \multicolumn{2}{c}{occupancy  $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} && \multicolumn{2}{c}{occupancy $\uparrow$}  && \multicolumn{2}{c}{collision $\downarrow$} && \multicolumn{2}{c}{occupancy $\uparrow$} \\
\cmidrule{4-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}\cmidrule{16-17}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       && \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline

\multirow{6}{*}{Decentralized} & \textsc{sparse}               && 0.482          & 0.450        && 0.594         & 0.627         && 0.946              & 1.170             && 0.015           & 0.107           && 0.042         & 0.091         \\
                               & \textsc{baseline}             && \textbf{0.522 }         & 0.394        && \textbf{0.617}         & \textbf{0.666}         && \textbf{1.028}              & 0.319             && 0.044           & \textbf{0.006}           && 0.044         & 0.045         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$           && 0.492          & \textbf{0.550 }       && 0.615         & 0.642         && 0.898              & 1.172             && 0.033           & 0.080          && 0.091         & 0.114         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$            && ---           & ---         && ---          & ---          && 0.955              & 1.146             && 0.013           & 0.065           && 0.182         & 0.080         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$          && ---           & ---        & & ---          & ---          && 0.890              & \textbf{1.294}             && 0.029           & 0.089           && 0.043         & 0.061         \\
                               & \textsc{shaped}             && 0.306          & 0.381        && 0.562         & 0.067         && 0.495              & 0.854             && \textbf{0.002}           & 0.018           && \textbf{1.026}         & \textbf{1.504}         \\\hline
\multirow{5}{*}{Centralized}   & \textsc{sparse}               && \textbf{0.479}          & 0.099        && 0.462         & 0.185        & & 0.825              & 0.492            & & 0.011           & 0.018           && 0.016         & 0.047         \\
                               & \textsc{baseline}  && 0.022          & 0.059        && \textbf{0.518}         & 0.255         && 0.887              & 0.458             && \textbf{0.001}           & 0.086           && 0.100         & 0.061         \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$           && 0.377          & \textbf{0.406}        && 0.490         & \textbf{0.443}         && 0.804              & 0.554             && 0.002           & 0.083           && 0.078         & 0.041         \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$            && ---           & ---         && ---          & ---          && \textbf{1.042}              & \textbf{0.573}             && \textbf{0.001}           & 0.083           && \textbf{0.321}         & 0.042         \\
                               & \textsc{shaped}            && 0.173          & 0.089        && 0.089         &     0.144          && 0.534              & 0.198             && \textbf{0.001}           & \textbf{0.012}           && 0.067         & \textbf{0.434}        
\end{tabular}
}
\end{table*}


\begin{table*}[t]
    \centering
     \caption{  \label{tab:po_metric_2} Agent-to-target (agt-target) and agent-to-adversary (agt-adv) distances averages across test episodes under \textit{partial} observability. Lower scores are better for agt-target ($\downarrow$), and higher scores are better for agt-adv ($\uparrow$). }
    \scalebox{0.85}{
    \begin{tabular}{llp{0.001pt}rrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{3}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{4-8}\cmidrule{10-17}
\multicolumn{2}{l}{Task}                && \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Phy decep.}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\multicolumn{2}{l}{Metric}                && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$}  && \multicolumn{2}{c}{agt-adv dist $\uparrow$} && \multicolumn{2}{c}{agt-target dist $\downarrow$} \\
\cmidrule{4-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}\cmidrule{16-17}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       && \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline

\multirow{6}{*}{Decentralized} & \textsc{sparse}               && \textbf{0.264}             & 0.238           && 0.251            & 0.201            && 0.260              & 0.240             && 1.439           & 2.134           && 1.483            & 2.863            \\
                               & \textsc{baseline}             && 0.387             & 0.405           && 0.258            & \textbf{0.191}            && \textbf{0.248}              & 0.537             && 1.167           & 2.482           && 1.514            & 3.293            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$           && 0.341             & 0.264           && 0.242            & 0.209            && 0.262              & 0.238             && 1.306           & 2.175           && 1.323            & 2.727            \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$            && ---              & ---            && ---             & ---             && 0.250              & 0.234             && 1.458           & 2.318           && 1.060            & 2.868            \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$          && ---              & ---            && ---             & ---             && 0.270              & \textbf{0.219}             && 1.420           & 2.127           && 1.485            & 3.121            \\
                               & \textsc{shaped}               && 0.333             & \textbf{0.224}          && \textbf{0.241}           & 0.735            && 0.369              & 0.262             && \textbf{1.925}           & \textbf{3.009}           && \textbf{0.572}            & \textbf{1.227}            \\\hline
\multirow{5}{*}{Centralized}   & \textsc{sparse}               && \textbf{0.349}             & 0.333           && 0.319            & 0.328            && 0.302              & 0.325             && 1.432           & 2.284           && 1.690            & 3.313            \\
                               & \textsc{baseline}  && 0.640             & 0.401           && \textbf{0.292}            & 0.300            && 0.271              & 0.397             && 1.655           & 2.174           && 1.269            & 3.045            \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$           && 0.376             & \textbf{0.235}           && \textbf{0.292}            & \textbf{0.238}            && 0.289              & 0.342             && 1.602           & 2.397           && 1.337            & 3.320            \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$            && ---              & ---            && ---             & ---             && \textbf{0.257}              & \textbf{0.305}             && 1.572           & 2.510          && \textbf{1.053}            & 3.289            \\
                               & \textsc{shaped}               && 0.414             & 0.351           && 0.351            &             0.352     && 0.346              & 0.534            & & \textbf{1.821}           & \textbf{2.987}           && 1.293            & \textbf{2.055}           
\end{tabular}
}
   
\end{table*}


==> tables/po_test_reward.tex <==
\begin{table*}[t]
\centering 
\caption{\label{tab:po_test_reward}We report test episode extrinsic rewards under partial observability. With both centralized and decentralized algorithms, $\textrm{\textsc{elign}}_\textrm{team}$ outperforms all reward comparisons on all but one cooperative task (\textit{Heterogeneous navigation}, 4v0). On competitive settings, either  $\textrm{\textsc{elign}}_\textrm{team}$ and $\textrm{\textsc{elign}}_\textrm{adv}$ always exceeds \textsc{sparse}, mostly surpasses \textsc{baseline} and outperforms \textsc{shaped}. 
Importantly, the decentralized algorithm with $\textrm{\textsc{elign}}_\textrm{team}$ outperforms the centralized algorithm with $\textrm{\textsc{shaped}}$ on all but one task (\textit{predator-prey}). This demonstrates the benefit of using alignment as intrinsic reward to train better decentralized policies that outperform centralized with domain-specific rewards.
}
\scalebox{0.81}{
\begin{tabular}{llrrp{0.001pt}rr p{0.001pt} rrp{0.001pt}rrp{0.001pt}rr}
\multicolumn{2}{l}{}                & \multicolumn{5}{c}{Cooperative}                              & & \multicolumn{8}{c}{Competitive}                                                                            \\
\cmidrule{3-7}\cmidrule{9-16}
\multicolumn{2}{l}{Task}                & \multicolumn{2}{c}{Coop nav.} && \multicolumn{2}{c}{Heter nav.} && \multicolumn{2}{c}{Physical deception}  && \multicolumn{2}{c}{Predator-prey} && \multicolumn{2}{c}{Keep-away} \\
\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}\cmidrule{15-16}
\multicolumn{2}{l}{Agt \# vs. Adv \#}       & \multicolumn{1}{c}{3v0}           & \multicolumn{1}{c}{5v0}          && \multicolumn{1}{c}{4v0}           & \multicolumn{1}{c}{6v0}     && \multicolumn{1}{c}{2v1}                & \multicolumn{1}{c}{4v2}               && \multicolumn{1}{c}{2v2}             & \multicolumn{1}{c}{4v4}             && \multicolumn{1}{c}{2v2}           & \multicolumn{1}{c}{4v4}           \\\hline
\multirow{6}{*}{Decentralized} & \textsc{sparse}              & 130.999       & 438.587      && 281.750       & 574.314       && 94.521             & 195.995           && -5.512          & -27.011         && 1.300         & -0.900        \\
                               & \textsc{baseline}            & 152.385       & 514.697      && 289.543       & 545.050       && 53.583             & 161.945           && -16.179         & \textbf{-0.354}          && 5.500         & -4.000        \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$          & \textbf{155.351 }      & \textbf{517.335}      && \textbf{302.380}       & \textbf{590.390}       && \textbf{97.985}             & 236.084          && -12.194         & -25.285         && 5.598         & \textbf{1.853}        \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$          & ---          & ---        && ---          & ---          && 95.500             & 234.210           && -4.125          & -17.569         && 27.295        & 1.833         \\
                               & $\textrm{\textsc{elign}}_\textrm{both}$         & ---          & ---         && ---          & ---          && 87.703             & 193.198           && -4.333          & -25.746         && 2.172         & -8.119        \\
                               & \textsc{shaped}               & 112.812       & 299.824      && 148.753       & 124.754       && 28.000             & \textbf{282.000}           && \textbf{-0.521}          & -6.056          && \textbf{40.344}        & -41.201       \\\hline
\multirow{5}{*}{Centralized}   & \textsc{sparse}              & 120.947       & 123.012      && 150.374       & 307.847       && 94.705             & -36.000           && -8.415          & -7.338         && -0.500        & -8.821        \\
                               & \textsc{baseline}  & 137.382       & 46.147       && \textbf{216.453}       & 279.257       && 104.374            & 20.874            && \textbf{-0.096}          & -25.700         && 4.000         & -4.225        \\
                               & $\textrm{\textsc{elign}}_\textrm{team}$          & \textbf{139.578}       & \textbf{178.212}      && 186.877       & \textbf{314.882}       && \textbf{107.912}            & \textbf{114.958}           && -0.178          & -31.425         && 6.348         & -4.000        \\
                               & $\textrm{\textsc{elign}}_\textrm{adv}$          & ---          & ---         && ---          & ---          && 77.149             & 59.555            && -0.271          & -24.331         && \textbf{28.000}        & \textbf{1.000}         \\
                               & \textsc{shaped}              & 81.094        & 88.628       && 73.057        & 297.623             && 79.520             & 7.197             && -1.123          & \textbf{-4.740}          && -11.750       & -43.194      
\end{tabular}
}
\end{table*}
